Leveraging 3D Information in Unsupervised Brain MRI Segmentation

Automatic segmentation of brain abnormalities is challenging, as they vary considerably from one pathology to another. Current methods are supervised and require numerous annotated images for each pathology, a strenuous task. To tackle anatomical variability, Unsupervised Anomaly Detection (UAD) methods are proposed, detecting anomalies as outliers of a healthy model learned using a Variational Autoencoder (VAE). Previous work on UAD adopted a 2D approach, meaning that MRIs are processed as a collection of independent slices. Yet, it does not fully exploit the spatial information contained in MRI. Here, we propose to perform UAD in a 3D fashion and compare 2D and 3D VAEs. As a side contribution, we present a new loss function guarantying a robust training. Learning is performed using a multicentric dataset of healthy brain MRIs, and segmentation performances are estimated on White-Matter Hyperintensities and tumors lesions. Experiments demonstrate the interest of 3D methods which outperform their 2D counterparts.

==> datasets.tex <==

\subsection{Datasets}
\label{sssec:Datasets}
We constituted our training dataset by pooling FLAIR data from several healthy datasets, as shown in Table \ref{table:methods}. In total, 79 healthy FLAIR MRI scan were collected.

\begin{center}
\begin{tabular}{|>{\centering}m{2.7cm}|>{\centering}m{3cm}|} \hline
    \textbf{Dataset}  &  \textbf{Number of scan}
    \tabularnewline \hline
    ADNI3  \cite{weiner2013alzheimer} & 20
    \tabularnewline \hline
    IBC  \cite{pinho2018individual} & 12
    \tabularnewline \hline
    Kirby \cite{landman2011multi} & 21
    \tabularnewline \hline
    Pixyl & 26  
    \tabularnewline \hline
    \textbf{Total} & 79
    \tabularnewline \hline
\end{tabular}
\captionof{table}{Composition of the training dataset}
\label{table:methods}
\end{center}

% We collected 20 scans from the Control Normal group of the ADNI3 dataset \cite{ADNI}, 12 scans from the IBC dataset \cite{IBC2018} and 21 scans from the Kirby dataset \cite{Kirby}. Finally, 26 scans from an inhouse dataset were collected, resulting in a total of 79 FLAIR scans. 

To evaluate the performance of our networks on UAD, an inhouse MS dataset was used composed of 196 subjects obtained from more than 20 centers. Both training and testing scans were preprocessed using a registration to a 170 x 192 x 170 reference template, followed by N4 bias correction and histogram normalization \cite{nyul1999standardizing}. Finally, intensities were normalized into the range [0,1] and skull-stripped. For 2D models, 75 axial slices around the central slice were extracted for each scan in order to remove irrelevant slices without brain, susceptible to disrupt training. 

